TransEditor: Transformer-Based Dual-Space GAN for Highly Controllable Facial Editing

Recent advances like StyleGAN have promoted the growth of controllable facial editing. To address its core challenge of attribute decoupling in a single latent space, attempts have been made to adopt dual-space GAN for better disentanglement of style and content representations. Nonetheless, these methods are still incompetent to obtain plausible editing results with high controllability, especially for complicated attributes. In this study, we highlight the importance of interaction in a dual-space GAN for more controllable editing. We propose TransEditor, a novel Transformer-based framework to enhance such interaction. Besides, we develop a new dual-space editing and inversion strategy to provide additional editing flexibility. Extensive experiments demonstrate the superiority of the proposed framework in image quality and editing capability, suggesting the effectiveness of TransEditor for highly controllable facial editing.

==> Arxiv/05_ablation.tex <==

\section{Ablation Study}
To highlight the contribution of different components in our model, we compare TransEditor with several other ablated models with various settings. 

\subsection{Space Interaction via Transformer}

\iffalse
\begin{figure*}
  \centering
  % \begin{minipage}{.45\textwidth}
  \begin{minipage}{0.45\linewidth}
    %\centering
    \begin{subfigure}{0.22\linewidth}
    \includegraphics[height=3cm, width=3cm]{figures/select_ablation_swap.png} 
    \caption{Z as Q matrix, P as K,V matrix}
    \label{fig:z-as-q p-k-v}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.22\linewidth}
    \includegraphics[height=3cm, width=3cm]{figures/select_ablation_swap_origin.png}
    \caption{P as Q matrix, Z as K,V matrix}
    \label{fig:p-as-q z-k-v}
  \end{subfigure}\hfill
  \label{fig:ablation-kqv}
  \end{minipage}
    \begin{minipage}{.45\textwidth}
  %\begin{subfigure}{0.475\linewidth}
    \centering
    {\includegraphics[width=4cm]{./figures/edit_ablation.pdf}}
    \captionof{figure}{Ablation}
    \label{fig:ablation-edit}
    
    \caption{Example of different choice for Q,K,V matrix.}
  \end{minipage}
  %\end{subfigure}
  \end{figure*}
\fi

\begin{figure}[]
  \centering
    \includegraphics[width=0.49\textwidth]{./figures/edit_ablation.pdf}
    \caption{\textbf{Ablation Study on Transformer and Dual-space}. Three rows represent editing result of head pose using TransEditor minus dual space, TransEditor minus Transformer and TransEditor itself, respectively.}
  \label{fig:ablation-edit}
 \end{figure}



\begin{figure}
  \centering

    \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/select_ablation_swap.png} 
    \caption{Z as Q matrix, P as K,V matrix}
    \label{fig:z-as-q p-k-v}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/select_ablation_swap_origin.png}
    \caption{P as Q matrix, Z as K,V matrix}
    \label{fig:p-as-q z-k-v}
  \end{subfigure}
  \label{fig:ablation-kqv}
  \caption{\textbf{Ablation study on different interaction method using Transformer.} Both images are generated by fixing $\bm{z}$ code and swapping p code at each column. Figure(b) is the our current setting, which shows a more disentangled result than figure(a).}
   
  \iffalse
  \begin{minipage}{.45\linewidth}
  \begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\textwidth]{./figures/edit_ablation.pdf}
    \end{subfigure}
    \end{minipage}
  \fi
  \end{figure}
  









The space interaction is crucial in our architecture for the semantic balance between the two spaces. Removing the interaction process, \ie. the generator will receive two completely independent codes compared with our design that the $\mathcal{Z}$-space is adopted to the $\mathcal{P}$-space, will result in an unbalanced result. Under this setting,  the generated images are mostly controlled by the $\mathcal{P}$-space, \ie.,the style information such as hue is also contained in the $\mathcal{P}$-space. In the first row of ~\cref{fig:ablation-edit}, we show the editing result of pose without the cross-space attention. We observe that the edited images suffer from severe face deformation with the step size of pose editing increasing, since the $\mathcal{P}$-space controls the majority of the information which is more entangled. In contrast, with added the cross-space interaction mechanism, the tones of the image can keep consistent during pose editing (Row 3, ~\cref{fig:ablation-edit}). Therefore, establishing a connection between the two spaces enables a more balanced setting, which benefits attribute editing.


\subsection{Dual Space Design v.s. Single Space Design}
We then evaluate the role of the dual space design. TransStyleGAN~\cite{vaswani2017attention} also makes use of the self-attention mechanism to establish connections between different style codes within the single space design. However, as can be seen in the second row of ~\cref{fig:ablation-edit}, when the step size of editing pose gets larger, the face orientation is still difficult to change, while the distortion of the face and the change of tone could be serious. This reflects the difficulty of editing pose in single space and demonstrates the advantage of our dual latent spaces.


\subsection{Selection of K, Q, V matrices}\label{ablation_kqv}
Due to the dual space design, we need to consider the choice the $\mathbf{K}, \mathbf{Q}, \mathbf{V}$ matrices for cross-space attention.

Some works in the multi-modal field utilize the single-modality feature that needs to be refined as the query, and the other modality feature as the key and value. %Then the refined features and the input single-modality feature will be residually connected. 
In our case, this is equivalent to using the $\bm{z}^{+}$ space as the query matrix and the $\bm{p}^{+}$ space as the key and value matrix. However, the output of the cross-space attention module, as the refined feature of the $\bm{z}^{+}$ space, is a weighting of the value matrix ($\bm{p}^{+}$ space), which inevitably produces the entanglement of the two spaces. This setting(\cref{fig:z-as-q p-k-v}) shows a severe entanglement between $\mathcal{P}$-space and $\mathcal{Z}$-space that swapping $\bm{p}$ codes will result in different textures, 
which is not desirable for editing. On the other hand, our setting shown in \cref{fig:p-as-q z-k-v} is better disentangled, since the $\bm{p}^{+}$ space is only adopted to as query to help update the $\bm{z}^{+}$ space. Therefore, this interaction method in \cref{Transformer-based Cross-space Interaction} is optimal for our design. 
% 
%Therefore, we modified this generic paradigm. To be more specific, our model only use the \(p^{+}\) space as the query matrix, and the \(z^{+}\) space will serve as key and value matrix. Meanwhile, the interaction result will be added with the the input \(z^{+}\) space feature in the subsequent residual connection. In this interaction setting, the \(p^{+}\) space is only used to help update the \(z^{+}\) space. Therefore, the updated Z-space features and the P-space features remain disentangled throughout the interaction process. As can be seen in Figure 9(b), when swapping the P-space code in each column, the texture keep consistent compared to the Figure 9(a).

% Each column of ~\cref{fig:ablation-kqv} is given by fixing Z-space code and randomly swap the P-space code. 

\iffalse
\subsection{Trials of training techniques}
The Path Regularization Loss given by StyleGAN2 is used to smooth the latent space w, which is minimized when changing a fixed step of the latent code will result in a fixed-magnitude change in the image. In our design, the space that corresponds to w in StyleGAN is the output of our cross-space interaction, as described in \cref{Transformer-based Cross-space Interaction}. Since it is not disable that any certain layer of the w space be dominant, we utilize the same regularization loss on our w space. 

We have also experimented to add the regularization loss on the \(p^{+}\) space. The result shows that this will discourage the \(p^{+}\) to influence the final result. When this regularization loss is added, changing the entire P-space code will only affect a little change in the image, which is undesirable since we need more balanced dual spaces for editing. 
\fi


\iffalse
\section{Ablation Study}
To highlight the contribution of different components in our model, we compare TransEditor against several other ablated models with various settings. 

\subsection{Space Interaction via Transformer}

\begin{figure*}
  \centering
  % \begin{minipage}{.45\textwidth}
  \begin{minipage}{0.45\linewidth}
    %\centering
    \begin{subfigure}{0.22\linewidth}
    \includegraphics[height=3cm, width=3cm]{figures/select_ablation_swap.png} 
    \caption{Z as Q matrix, P as K,V matrix}
    \label{fig:z-as-q p-k-v}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.22\linewidth}
    \includegraphics[height=3cm, width=3cm]{figures/select_ablation_swap_origin.png}
    \caption{P as Q matrix, Z as K,V matrix}
    \label{fig:p-as-q z-k-v}
  \end{subfigure}\hfill
  
  \end{minipage}
    \begin{minipage}{.45\textwidth}
  %\begin{subfigure}{0.475\linewidth}
    \centering
    {\includegraphics[width=4cm]{./figures/edit_ablation.pdf}}
    \captionof{figure}{Ablation}
    \label{fig:ablation-edit}
    
    \caption{Example of different choice for Q,K,V matrix.}
  \end{minipage}
  %\end{subfigure}
  \end{figure*}

The space interaction is crucial in our architecture for the semantic balance between the two spaces. Removing the interaction process, \ie the generator will receive two completely independent codes compared with our design that the Z-space is adopted to the P-space, will result in an unbalanced result. We found that the generated images are mostly controlled by the P-space(the initial feature map), \ie, the P-space also controls the style information such as hue. In the first row of Figure 8, we show the editing result of pose without the cross-space attention. We can observe that when the step size of pose editing is gradually increased, the image will suffer from serious tonal changes, due to the P-space also controlling the tonal information. In contrast, the tones of the image can keep consistent when we edit the pose attribute, which proves that the cross-space interaction mechanism we proposed can establish a connection between the two spaces and make these two spaces more balanced for better attribute editing.

\subsection{Dual Space Design v.s. Single Space Design}
We then evaluate the role of the dual space design. TransStyleGAN~\cite{vaswani2017attention} also makes use of the self attention mechanism to establish connections between different style codes within the single space design. However, as can be seen in the second row of Figure 9, when the step size of editing pose is larger, the face orientation is still difficult to change. At the same time, as the step size increases, the distortion of the face and the change of tone can be serious. 

\subsection{Selection of K, Q, V matrices}
Due to the dual space design, we need to consider which space to use as the query matrix and the other as the key and value matrix for cross-space attention. In some work in the multi-modal field, they usually use the single-modality feature that need to be refine \chengyao{refined} as query matrix and the other modality feature as the key and value matrix. Then the refined features and the input single-modality feature will be residually connected. 

We also tried this setting, using the \(z^{+}\) space as the query matrix and the \(p^{+}\) space as the key and value matrix. However, the output of the cross-space attention module, as the refined feature of the \(z^{+}\) space, is a weighting of the value matrix(\(p^{+}\) space). This weighting method inevitably produces the entanglement of the two spaces, as the updated \(z^{+}\) space feature vector is a linear combination of \(z^{+}\) space feature vectors. We show the visualization results of this setting in Figure 9(a). In each column, we fix Z-space code and randomly swap the P-space code. The figure shows that swapping P-space codes will result in different textures. This implies a severe entanglement between P-space and z-space which is not what we expect. Therefore, we modified this generic paradigm. To be more specific, our model only use the \(p^{+}\) space as the query matrix, and the \(z^{+}\) space will serve as key and value matrix. Meanwhile, the interaction result will be added with the the input \(z^{+}\) space feature in the subsequent residual connection. In this interaction setting, the \(p^{+}\) space is only used to help update the \(z^{+}\) space. Therefore, the updated Z-space features and the P-space features remain disentangled throughout the interaction process. As can be seen in Figure 9(b), when swapping the P-space code in each column, the texture keep consistent compared to the Figure 9(a).


\subsection{Trials of training techniques}
The Path Regularization Loss given by StyleGAN2 is used to smooth the latent space w, which is minimized when changing a fixed step of the latent code will result in a fixed-magnitude change in the image. In our design, the space that corresponds to w in StyleGAN is the output of our cross-space interaction, as described in section 3.2. Since we do not want any certain layer of the w space to be dominant, we utilize the same regularization loss on our w space. 

We have also experimented to add the regularization loss on the \(p^{+}\) space. The result shows that this will discourage the \(p^{+}\) to influence the final result. When this regularization loss is added, changing the entire P-space code will only affect a little change in the image, which is undesirable since we need more balanced dual spaces for editing.   
\fi

% The layer-wise noise is used as the stochastic variation during the generation process of StyleGAN. In our architecture, we have also trained the generator network with and without layer-wise noise. Adding the noise would help reducing the FID score further, yet the PPL will increase vastly. We think since the interaction of our network occurs before the generating process, adding the noise will influence the interaction process.

\iffalse
\subsection{Number of Transformer}
The number of Transformer layers is correlated with the degree of interaction. When the number of layers gets larger, the \(s^{+}\) code will be more adopted \chengyao{what dose adopted mean?} to the \(p^{+}\) code used for interaction. We experimented on different number of Transformer, and using more layers will result in better head pose consistency when \(p^{+}\) code is fixed, although the difference is not that significant. In most of our settings, we utilize 8 layers of Transformers. 
\fi

